Pulsar Timing Arrays: Status and Techniques

Three pulsar timing arrays are now producing high quality data sets. As reviewed in this paper, these data sets are been processed to 1) develop a pulsar-based time standard, 2) search for errors in the solar system planetary ephemeris and 3) detect gravitational waves. It is expected that the data sets will significantly improve in the near future by combining existing observations and by using new telescopes.

==> PaxHeader/hobbs.tex <==
14 gid=286816
20 ctime=1349823138
20 atime=1349823140
24 SCHILY.dev=234881026
23 SCHILY.ino=13747623
18 SCHILY.nlink=1

